"Why did the Model Fail?": Attributing Model Performance Changes to Distribution Shifts

Machine learning models frequently experience performance drops under distribution shifts. The underlying cause of such shifts may be multiple simultaneous factors such as changes in data quality, differences in specific covariate distributions, or changes in the relationship between label and features. When a model does fail during deployment, attributing performance change to these factors is critical for the model developer to identify the root cause and take mitigating actions. In this work, we introduce the problem of attributing performance differences between environments to distribution shifts in the underlying data generating mechanisms. We formulate the problem as a cooperative game where the players are distributions. We define the value of a set of distributions to be the change in model performance when only this set of distributions has changed between environments, and derive an importance weighting method for computing the value of an arbitrary set of distributions. The contribution of each distribution to the total performance change is then quantified as its Shapley value. We demonstrate the correctness and utility of our method on synthetic, semi-synthetic, and real-world case studies, showing its effectiveness in attributing performance changes to a wide range of distribution shifts.

==> paper_arXiv/convergence_analysis.tex <==
\section{Convergence Analysis}
\label{app:convergence}

We present a preliminary analysis to study the impact of errors resulting from estimating importance weights on the properties of the Shapley values. The theoretical analysis is informal and presented here with the goal of motivating further study. Importantly, we experimentally evaluate the error in a synthetic setup.

\subsection{Sketch for a Theoretical Analysis}














\begin{remark}
    Under bounded estimation error and for a bounded loss, Property 2.1 holds asymptotically.
\end{remark}

\begin{proof}
    Suppose $ 1 - \epsilon_d^n \leq  w_d \leq 1 + \epsilon_d^n$, that is we get approximate importance weights from finite samples. Then for a bounded loss,
    \begin{equation}
        \begin{aligned}
           - \frac{\epsilon_{d}^n l}{|\cand|} \sum_{\subcand\subseteq \cand \setminus \{d\}} \binom{|\cand| - 1}{|\subcand|}^{-1} \mathbb{E}_{\psrc}[\prod_{\tilde{d} \in \subcand \cup d} w_{\tilde{d}}]  \leq \text{Attr}^n(d)  \leq \frac{\epsilon_d^n l}{|\cand|} \sum_{\subcand\subseteq \cand \setminus \{d\}} \binom{|\cand| - 1}{|\subcand|}^{-1} \mathbb{E}_{\psrc}[\prod_{\tilde{d} \in \subcand \cup d} w_{\tilde{d}}]
        \end{aligned}
    \end{equation}

    Suppose that in the worst case all other distributions shift except $d$, but the shifts are bounded, i.e.  $\frac{1}{\eta} < w_{\tilde{d}} < \eta$ where $\eta>1$ for all $\tilde{d} \in \cand \setminus \{d\}$. Then,
    \begin{equation}
        \begin{aligned}
        &- \frac{\epsilon_{d}^n l}{|\cand|} \sum_{\subcand\subseteq \cand \setminus \{d\}} \binom{|\cand| - 1}{|\subcand|}^{-1} \left(\frac{1}{\eta}\right)^{|\subcand| - 1}  \leq \text{Attr}^n(d)  \leq \frac{\epsilon_d^n l}{|\cand|} \sum_{\subcand\subseteq \cand \setminus \{d\}} \binom{|\cand| - 1}{|\subcand|}^{-1} {\eta}^{|\subcand| - 1} \\
        & - \frac{\epsilon_{d}^n l}{|\cand|} \left(1 + \frac{1}{\eta}\right)^{|\subcand| - 1}  \leq \text{Attr}^n(d)  \leq \frac{\epsilon_d^n l}{|\cand|}  {(1+\eta)}^{|\subcand| - 1}
        \end{aligned}
        \end{equation}

        The error in attribution is dominated by the shifts in other distribution and the error in estimating the weight for distribution $d$. Thus as $n \to \infty$, so long as $\epsilon_d^n \to 0$, the attribution $\text{Attr}^n(d) \to 0$. 
\end{proof}
The above suggests that our Property 2.1 may not hold exactly in finite samples due to estimation error.



    
    






    




\subsection{Empirical Analysis}
To empirically examine the estimation error as a function of the number of samples, we adopt the synthetic setup described in Appendix \ref{app:synthetic} with 
$\theta_2 = 0.5$ and $\mu_2 = 0.5$. We choose this setup because the exact importance weights can be computed analytically, and thus allows us to quantify the error of an importance weight estimator. We experiment with the KLIEP method \cite{sugiyama2008direct}, as well as using logistic regression (LR) and XGBoost (XGB) as probabilistic estimators, the last of which we use in the paper. Given $n$ samples, we randomly choose $n/2$ samples to train the importance weight estimator, and the remaining $n/2$ samples to evaluate the attribution. In each run, we compute the mean squared error between empirical and exact importance weights for 
$\cD_X$ and $\cD_{Y|X}$, as well as the mean squared error between the empirical and exact attributions $Attr(\cD_X)$ and $Attr(\cD_{Y|X})$. Note that the analytical attributions are 
$Attr(\cD_X) = -0.06375$ and 
$Attr(\cD_{Y|X}) = 0.16875$. We display the result in Table \ref{tab:convergence}.

\begin{table}[!ht]
    \centering
    \caption{Estimation error in Shapley attributions for finite samples, using the synthetic setup described in Appendix \ref{app:synthetic}.}
    \begin{tabular}{lrrrrr}
    \toprule
        \textbf{Model} & $n$ & $MSE(w_X)$ & $MSE(w_{X, Y})$ & $MSE(Attr(\cD_X))$ & $MSE(Attr(\cD_Y))$ \\ 
        \midrule
        \multirow{ 3}{*}{KLIEP} & 100 & 0.557 $\pm$ 0.339 & 1.093 $\pm$ 0.422 & 0.016 $\pm$ 0.003 & 0.029 $\pm$ 0.015 \\ 
         & 200 & 0.344 $\pm$ 0.194 & 1.612 $\pm$ 0.809 & 0.004 $\pm$ 0.000 & 0.037 $\pm$ 0.002 \\ 
         & 1000 & 0.212 $\pm$ 0.145 & 0.588 $\pm$ 0.203 & 0.003 $\pm$ 0.001 & 0.041 $\pm$ 0.012 \\ \midrule
        \multirow{8}{*}{LR} & 20 & 0.237 $\pm$ 0.133 & 0.428 $\pm$ 0.221 & 0.004 $\pm$ 0.000 & 0.028 $\pm$ 0.000 \\ 
         & 50 & 0.748 $\pm$ 0.707 & 14.175 $\pm$ 22.402 & 0.004 $\pm$ 0.000 & 0.023 $\pm$ 0.005 \\ 
         & 100 & 0.555 $\pm$ 0.064 & 0.549 $\pm$ 0.342 & 0.004 $\pm$ 0.000 & 0.033 $\pm$ 0.009 \\ 
         & 200 & 0.543 $\pm$ 0.083 & 1.861 $\pm$ 1.864 & 0.004 $\pm$ 0.000 & 0.036 $\pm$ 0.012 \\ 
         & 1000 & 0.600 $\pm$ 0.042 & 4.549 $\pm$ 3.196 & 0.004 $\pm$ 0.000 & 0.010 $\pm$ 0.007 \\ 
         & 5000 & 0.583 $\pm$ 0.061 & 3.208 $\pm$ 0.269 & 0.004 $\pm$ 0.000 & 0.008 $\pm$ 0.003 \\ 
         & 10000 & 0.566 $\pm$ 0.038 & 5.887 $\pm$ 3.753 & 0.004 $\pm$ 0.000 & 0.007 $\pm$ 0.004 \\ 
         & 50000 & 0.325 $\pm$ 0.008 & 3.631 $\pm$ 0.430 & 0.004 $\pm$ 0.000 & 0.009 $\pm$ 0.002 \\  \midrule
        \multirow{8}{*}{XGB} & 20 & 1.191 $\pm$ 1.034 & 0.974 $\pm$ 0.740 & 0.003 $\pm$ 0.003 & 0.068 $\pm$ 0.038 \\ 
         & 50 & 1.003 $\pm$ 0.848 & 40.087 $\pm$ 66.979 & 0.010 $\pm$ 0.008 & 0.022 $\pm$ 0.004 \\ 
         & 100 & 13.151 $\pm$ 19.926 & 30.083 $\pm$ 25.079 & 0.017 $\pm$ 0.016 & 0.013 $\pm$ 0.020 \\ 
         & 200 & 10.053 $\pm$ 8.450 & 7.491 $\pm$ 9.321 & 0.001 $\pm$ 0.001 & 0.031 $\pm$ 0.015 \\ 
         & 1000 & 0.418 $\pm$ 0.378 & 39.845 $\pm$ 66.373 & 0.005 $\pm$ 0.003 & 0.031 $\pm$ 0.023 \\ 
         & 5000 & 0.419 $\pm$ 0.502 & 3.485 $\pm$ 2.964 & 0.003 $\pm$ 0.003 & 0.030 $\pm$ 0.025 \\ 
         & 10000 & 0.065 $\pm$ 0.062 & 0.903 $\pm$ 0.429 & 0.001 $\pm$ 0.001 & 0.014 $\pm$ 0.018 \\ 
         & 50000 & 0.083 $\pm$ 0.050 & 0.396 $\pm$ 0.095 & 0.000 $\pm$ 0.000 & 0.002 $\pm$ 0.001 \\ 
        \bottomrule
    \end{tabular}
    \label{tab:convergence}
\end{table}

We first find that KLIEP did not converge for smaller values of 
$n$, and takes prohibitively long to run for larger values of 
$n$. It was for these reasons that we did not select it for use in the main paper. Next, we note that a linear model is not complex enough to differentiate between the source and target, and thus results in a biased estimator (non-zero MSE for large n), though this still results in relatively small MSE for the attributions. Finally, we observe that the errors of XGB converge to zero both in the estimated importance weights as well as in the resulting attributions.

==> paper_arXiv/method.tex <==
\section{Problem Setup}\label{sec:preliminaries}

\textbf{Notation.} Consider a learning setup where we have some system variables denoted by $V$ consisting of two types of variables $V=(X,Y)$, which comprises of features $X$ and labels $Y$ such that $V \sim \cD$. Realizations of the variables are denoted in lower case. We assume access to  samples from two environments. We use $\psrc$ to denote the source distribution and $\ptar$ for the target distribution. Subscripts on $\cD$ refer to the distribution of specific variables. For example, $\cD_{X_1}$ is the distribution of feature $X_1 \subset X$, and $\cD_{Y| X}$ is the conditional distribution of labels given all features $X$. 

Let $X_{\texttt{M}} \subseteq X$ be the subset of features utilized by a given model $f$. We are given a loss function $\ell((x,y), f) \mapsto  \reals$ which assigns a real value to the model evaluated at a specific setting  $x$ of the variables. For example, in the case of supervised learning, the model $f$ maps $X_{\texttt{M}}$ into the label space, and a loss function such as the squared error $\ell((x,y),f) := (y-f(x_{\texttt{M}}))^2$ can be used to evaluate model performance. We assume that the loss function can be computed separately for each data point. Then, performance of the model in some environment with distribution $\cD$ is summarized by the average of the losses:
\begin{equation*}
 \perf(\cD) := \E_{(x, y)\sim \cD} [\ell((x, y), f)]   
\end{equation*}
This implies that a shift in any variables $V$ in the system may result in performance change across environments, including those that are not directly used by the model, but drive changes to the features $X_{\texttt{M}}$ used by the model for learning.

{\textbf{Setup.}} Suppose we are given a \textit{candidate set} of (marginal and/or conditional) distributions  $\cand$ over $V$ that may account for the model performance change from $\psrc$ to $\ptar$: $\perf(\ptar) - \perf(\psrc)$. %
\textbf{Our goal is to attribute this change to each distribution in the candidate set $\cand$.} %
For our method, we assume access to the model $f$, and samples from $\psrc$ as well as  $\ptar$ (see Figure~\ref{fig:example}).

We assume that dependence between variables $V$ is described by a causal system~\cite{pearl2009causality}. For every variable $X_i \in V$, this dependence is captured by a functional relationship between $X_i$ and the so-called ``causal parents'' of $X_i$ (denoted as $\text{parent}(X_i)$) driving the variation in $X_i$. The causal dependence induces a Markov distribution over the variables in this system. That is, the joint distribution $\cD_V$ can be factorized as, $\cD_V = \prod_{X_i \in V} \cD_{X_i | \text{parent}(X_i)}$. This dependence can be summarized graphically using a Directed Acyclic Graph (DAG) with nodes corresponding to the system variables and directed edges ($\text{parent}(X_i) \rightarrow X_i$) in the direction of the causal mechanisms in the system (see Figure~\ref{fig:example} for an example).

\textbf{Example.} We provide an example that illustrates that the performance attribution problem is ill-specified without knowing how the mechanisms can change to result in the observed performance difference. Suppose we are predicting $Y$ from $X$ with a linear model $f(x):=\phi x$ under the squared loss function. Consider two possible scenarios for data generation -- (1) $X\leftarrow Y$ where $\cD_{Y}$ changes from source to target while $\cD_{X|Y}$ remains the same, (2) $X\rightarrow Y$ where $\cD_{X}$ changes from source to target while $\cD_{Y|X}$ remains the same. The performance difference of $f(x)$ is the same in both the cases. Naturally, we want an attribution method to  assign all of the difference to the mechanism for $Y$ in the first case and to the mechanism of $X$ in the second case. Thus, for the same performance difference between source and target data, we would like a method to output different attributions depending on whether the data generating process is case (1) or (2). Note that, in general, it is impossible to find the appropriate attributions by first finding the direction of the causal mechanisms. This follows from the fact that learning the structure is in general, impossible purely from observational data~\citep{peters2017elements}. Hence knowledge of the data-generating mechanisms is necessary for appropriate attribution.

More concretely, suppose the processes are (1) $Y\sim N(\mu_1,1), X\sim Y+N(0,1)$. The mean of $Y$ shifts to $\mu_2$ in target, and (2) $X\sim N(\mu_1,1), Y\sim X+N(0,1)$ where the mean of $X$ shifts to $\mu_2$ in target. For the model $f(x):=\phi x$, the performance difference $\Delta$ in both cases is $(1-\phi)^2(\mu_2^2-\mu_1^2)$. This example illustrates the need for specifying how the mechanisms can shift from source to target to solve the attribution problem. In this work, we use partial causal knowledge, {\bf{in terms of the causal graph only}}, to specify the data-generating mechanisms.

In general, this partial knowledge further allows us to identify potential shifts to consider. Specifically, the number of marginal and conditional shifts that can be defined over $(X,Y)$ is exponential in the dimension of $X$. The factorization induced by the causal graph or equivalently knowledge of the data-generating mechanism reduces the space of possible shifts to consider for attribution. See Section~\ref{sec:method} for additional advantages of using a causal framework. %













\section{Method}\label{sec:method}

We now formalize our problem setup and motivate a game theoretic method for attributing performance changes to distributions over variable subsets (See Figure \ref{fig:example} for a summary).  We proceed with the following Assumptions.

\begin{assumption}\label{ass:graph_known}
The causal graph corresponding to the data-generating mechanism is known and all variables in the system are observed. Thus, the factorization of the joint distribution $\cD_V$ is known.
\end{assumption}

\begin{assumption}\label{ass:shifts_as_interventions}
Distribution shifts of interest are due to (independent) shifts in one or more factors of $\cD_V$.
\end{assumption}

Given these assumptions, we now describe our game theoretic formulation for attribution.  
\begin{figure}[t]
            \centering
            \includegraphics[width=0.5\textwidth]{figures/change_attr_method.drawio.png}
            \caption{\textbf{Sketch of the game theoretic attribution method.} Each causal mechanism is a player that, if present in the coalition, changes to the target distribution and, if absent, remains fixed at the source distribution. This defines the distribution of the resulting coalition $\widetilde{\cD}$. Performance on $\widetilde{\cD}$ is estimated using importance sampling from training data samples. After computing values for each possible coalition, Shapley value (Eq. \ref{eq:shapley}) gives the attribution to each player. Thus, we estimate the performance change under all possible ways to shift the mechanisms from source to target and use these to distribute the total performance change among the individual distributions.}
            \label{fig:method}
        \end{figure}
  

\subsection{Game Theoretic Distribution Shift Attribution}
We consider the set of candidate distributions $\cand$ as the   \textit{players} in our attribution game. A \textit{coalition} of any subset of players determines the distributions that are allowed to shift (from their source domain distribution to the target domain distribution), keeping the rest fixed. The \textit{value} for the coalition is the model performance change between the resulting distribution for the coalition and the training distribution. See Figure~\ref{fig:method} for an overview of the method.

\paragraph{Value of a Coalition.} 
Consider a coalition of distributions $\subcand \subseteq \cand$. This coalition implies a joint distribution over system variables $V$, where members in the coalition contribute their target domain distribution, and non-members contribute their source domain distribution:

\begin{equation}\label{eq:src_d}
\begin{split}
    \widetilde{\cD} = & \underbrace{\left(\prod_{i: \cD_{X_i | \pa(X_i)}\in \subcand}  \ptar_{X_i | \pa(X_i)} \right)}_{\text{Coalition}} \cdot \\ &  \quad \underbrace{\left( \prod_{i: \cD_{X_i | \pa(X_i)}\not\in \subcand} \psrc_{X_i | \pa(X_i)} \right)}_{\text{Not in Coalition}}
    \end{split}
\end{equation}
 

The above factorization follows from Assumptions~\ref{ass:graph_known} and~\ref{ass:shifts_as_interventions}. Note that the coalition only consists of distributions that are allowed to change across environments. All other relevant mechanisms are indeed fixed to the source distribution. We present an example of a coalition of two players in Figure \ref{fig:method}. The value of the coalition $\subcand$ with the coalition distribution $\widetilde{\cD}$ is now given by
\begin{equation}
    \label{eq:value}
     \val(\subcand) := \perf(\widetilde{\cD}) - \perf(\psrc)\\
\end{equation}
Thus, our assumptions  allow us to represent a factorization where only members of the coalition change, while all other mechanisms correspond to the source distribution. If we consider the change in performance for all combinatorial coalitions, we can estimate the total contribution of a specific distribution by aggregating the value for all possible coalitions a candidate distribution is a part of. This is exactly the Shapley value applied to a set of distributions. The Shapley value framework thus allows us to obtain the attribution of each player $d \in \cand$ using Equation \ref{eq:shapley}.

Abstractly, the Shapley values framework \citep{shapley1953value} is a game theoretic framework which assumes that there are $\noscriptcand := \{1, 2, \dots, n\}$ players in a co-operative game, achieving some total value (in our case, model performance change). We denote by $\val : 2^\noscriptcand \mapsto \reals$, the value for any subset of players, which is called a coalition. %
Shapley values correspond to the fair assignment of the value $\val(\noscriptcand)$ to each player $d \in \noscriptcand$. The intuition behind Shapley values is to quantify the change in value when a player (here, a distribution) enters a coalition. Since the change in model performance depends on the order in which players (distributions) may join the coalition, Shapley values aggregate the value changes over all permutations of $\noscriptcand$. Thus the Shapley attribution $\attr(d)$ for a player $d$ is given by:
\begin{equation}
    \label{eq:shapley}
    \attr(d) = \frac{1}{|\noscriptcand|} \sum_{\subcand\subseteq \noscriptcand \setminus \{d\}} \binom{|\noscriptcand| - 1}{|\subcand|}^{-1} \left( \val(\subcand \cup \{d\}) - \val(\subcand)\right)
\end{equation}

where we measure the change in model performance (denoted by Val) after adding $d$ to the coalition averaged over all potential coalitions involving $d$. The computational complexity of estimating Shapley values is  exponential in the number of players. Hence we rely on this exact expression only when the number of candidate distributions is small. That is, the causal graph induces a factorization that results in smaller candidate sets. For larger candidate sets, we use previously proposed approximation methods \citep{castro2009polynomial,lundberg2017unified, janzing2020feature} for reduced computational effort.

\paragraph{Choice of Candidate Distribution Shifts.} We motivate further the choice of candidate distributions that will inform the coalition. %
As mentioned before, without the knowledge of the causal graph, many heuristics for choosing the candidate sets are possible. For example, a  candidate set could be the set of all marginal distributions on each system variable, $\cand=\{\cD_{X_1},\cD_{X_2},\cdots\}$, or distribution of each variable after conditioning on the rest, $\cand=\{\cD_{X_1|V\setminus X_1},\cD_{X_2|V\setminus X_2},\cdots\}$. Since we have combinatorially many shifts that can be defined on subsets of $V=(X,Y)$, choosing candidate sets that would then inform the coalition is challenging.  %
The causal graph, on the other hand, specifies the factorization of the joint distribution into a set of distributions. %
We form the candidate set  constituting each distribution in this factorization. That is,
\begin{equation*}
    \cand = \{\cD_{X_1 | \pa(X_1)}, \cdots,\cD_{X_i | \pa(X_i)}, \cdots\}_{i=1,\cdots,|V|}
\end{equation*}
For a node without parents in the causal graph, the parent set can be empty, which reduces $\cD_{X_i|\text{parent}(X_i)}$ to the  marginal distribution of $X_i$. 
This choice of candidate set has three main advantages. First, it is \textit{interpretable} since the candidate shifts are specified by domain experts who constructed the causal graph. Second, it is \textit{actionable} since identifying the causal mechanisms most responsible for performance change can inform mitigating methods for handling distribution shifts \citep{subbaswamy2019preventing}. Third, it will lead to \textit{succinct} attributions due to the independence property. 

Consider the case where only one conditional distribution $\cD(X_i | \pa(X_i))$ changes across domains. This will result in a change in distributions of all descendants of $X_i$ (due to the above factorization). In this case, a candidate set defined by all marginals is not succinct, as one would attribute performance changes to all marginals of descendants of $X_i$. Instead, the candidate set determined by the causal graph will isolate the correct conditional distribution. 


Crucially, to compute our attributions, we need estimates of model performance under $\widetilde{\cD}$. Note that we only have model performance estimates under $\psrc$ and $\ptar$, but not for any arbitrary coalition where only a subset of the distributions have shifted. To estimate the performance of any coalition, we propose to use importance sampling. 



\subsection{Importance Sampling to Estimate Performance under a Candidate Distribution Shift}


\begin{assumption}\label{ass:support}
$\texttt{support}(\ptar_{X_i | \pa(X_i)}) \subseteq \texttt{support}(\psrc_{X_i | \pa(X_i)}) $ for all $\ptar_{X_i | \pa(X_i)} {\in} \cand$.
\end{assumption}


Importance sampling allows us to re-weight samples drawn from a given distribution, which can be $\psrc$ or $\ptar$, to simulate expectations for a desired distribution, which is the candidate $\widetilde{\cD}$ in our case. Thus, we re-write the value as
\begin{align}
    \val(\subcand) &= \perf(\widetilde{\cD}) - \perf(\psrc) \label{eq:val_def} \\
    &= \E_{(x, y)\sim \widetilde{\cD}} [\ell((x,y),f)] - \E_{(x,y)\sim \psrc} [\ell((x,y),f)] \nonumber\\
    &= \E_{(x,y)\sim \psrc} \left[\frac{\widetilde{\cD}((x,y))}{\psrc((x,y))}\ell((x,y),f)\right] \nonumber - \\ & \qquad \E_{(x,y)\sim \psrc} [\ell((x,y),f)] \nonumber
\end{align}
The importance weights are themselves a product of ratios of source and target distributions corresponding to the causal mechanisms in $\cand$ as follows:
\begin{equation}
\begin{split}
    w_{\subcand}((x,y)) &:= \frac{\widetilde{\cD}((x,y))}{\psrc((x,y))} = \prod_{d \in \subcand} \frac{\ptar_d((x,y))}{\psrc_d((x,y))} \\ &=: \prod_{d \in \subcand} w_{d} ((x,y)) %
\end{split}
\end{equation}
By Assumption \ref{ass:support}, we ensure that all importance weights are finite.

\paragraph{Computing Importance Weights.} 
There are multiple ways to estimate importance weights $w_d((x, y))$, which are a ratio of densities \citep{sugiyama2012density}. Here, we use a simple approach for density ratio estimation via training probabilistic classifiers as described in \citet[][Section 2.2]{sugiyama2012density}.

Let $D$ be a binary random variable, such that when $D=1, Z\sim \ptar_d(Z)$, and when $D=0, Z\sim \psrc_d(Z)$. Suppose $d = \cD_{X_i | \pa(X_i)}$, then $$w_d =\frac{\pr(D = 0 | \pa(X_i))}{\pr(D = 1| \pa(X_i))} \cdot \frac{\pr(D = 1 | X_i, \pa(X_i))}{\pr(D = 0 | X_i, \pa(X_i))}, $$ where each term is computed using a probabilistic classifier trained to discriminate data points from $\psrc$ and $\ptar$ from the concatenated dataset. We show the derivation of this equation in Appendix \ref{app:iw_deriv}. In total, we need to learn $\bigO(|\cand|)$ models for computing all importance weights. 






\subsection{Properties of Our Method}

Under perfect computation of importance weights, the Shapley attributions resulting from the performance-change game have the following desirable properties, which follow from the properties of Shapley values. We provide proofs of these properties in Appendix \ref{app:proof_property}.


\begin{asparaenum}
\item[] {\bf{Property 1. (Efficiency)}} $\displaystyle\sum_{d \in \cand} \attr(d) = \val(\cand) = \perf(\ptar) - \perf(\psrc)$ %

\item[] {\bf{Property 2.1. (Null Player)}} $\psrc_d = \ptar_d \implies \attr(d) = 0$.


\item[] {\bf{Property 2.2. (Relevance)}}  Consider a mechanism $d$. If $\perf(\subcand \cup \{d\}) = \perf(\subcand)$ for all $\subcand \subseteq \cand \setminus d$, then ${\attr(d) = 0}$. 

\item[] {\bf{Property 3. (Attribution Symmetry)}} Let $\attr_{\cD_1, \cD_2}(d)$ denote the attribution to some mechanism $d$ when $\cD_1 = \psrc$ and $\cD_2 = \ptar$. Then, $\attr_{\cD_1, \cD_2}(d) = -\attr_{\cD_2, \cD_1}(d) \ \forall d \in \cand$.
\end{asparaenum}



Thus, the method attributes the overall performance change only to distributions that actually change in a way that affects the specified performance metric. The contribution of each distribution is computed by considering how much they impact the performance if they are made to change in different combinations alongside the other distributions. %





\subsection{Analysis using a Synthetic Setting}
\label{sec:simple_syn}
We derive analytical expressions for  attributions in a simple synthetic case with the following data generating process.
\begin{equation*}
    \begin{aligned}
    \text{Source}:  X &\sim \mathcal{N}(\mu_1, \sigma_X^2) \\
    Y &\sim \theta_1 X + \mathcal{N} (0, \sigma_Y^2) \\
    \text{Target}: X &\sim \mathcal{N}(\mu_2, \sigma_X^2) \\
    Y &\sim \theta_2 X + \mathcal{N} (0, \sigma_Y^2)
    \end{aligned}
\end{equation*}


The model that we are investigating is $f(X) = \phi X$, and $l((x, y), f) = (y - f(x))^2$.

\begin{table*}[t]
    \centering
     \caption{Analytical expressions of the attributions for the synthetic case described in Section \ref{sec:simple_syn}. For the full derivation, see Appendix \ref{app:synthetic}.}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lll}
    \toprule
        & \textbf{Attr($\cD_X$)} & \textbf{Attr($\cD_{Y|X}$)} \\
        \midrule
        \textbf{Ours} & $(\frac{1}{2}\mu_2^2 - \frac{1}{2}\mu_1^2) ((\theta_2 - \phi)^2 + (\theta_1 - \phi)^2)$  &  $ (\sigma_X^2 + \frac{1}{2} \mu_1^2 + \frac{1}{2} \mu_2^2) ((\theta_2 - \phi)^2 - (\theta_1 - \phi)^2) $ \\
        \midrule
        \textbf{\citet{budhathoki2021distribution}} & $\frac{(\mu_2 - \mu_1)^2}{2\sigma_X^2}$ & $\frac{(\theta_2 - \theta_1)^2}{2 \sigma_Y^2} (\sigma_X^2 + \mu_2^2)$ \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:synthetic_expr}
\end{table*}


We show the attribution of our method, along with the attribution using the joint method from \citet{budhathoki2021distribution}, in Table \ref{tab:synthetic_expr}. The complete derivation, along with experimental verification of the derived expressions, can be found in Appendix \ref{app:synthetic}. We highlight several advantages that our method has over the baseline.

First, our attribution takes the model parameter $\phi$ into account in order to explain model performance changes, whereas~\citet{budhathoki2021distribution} do not, as they only explain shifts in $(X, Y)$, or changes in simple functions such as $\mathbb{E}[X]$ of the variables. Second, we find that our $\attr(\cD_X)$ is a function of $\theta_2$. This is desirable, as covariate shift may compound with concept shift to increase loss non-linearly. This also ensures that both attributions always sum to the total shift. Third, we note that our attributions are \textit{signed}, which is particularly important as some shifts may decrease loss. Finally, we note that our attributions are symmetric when the source and target data distributions are swapped by Property 3. This is not true of the baseline method in general, as the KL divergence is asymmetric. Since we assume knowledge of the true causal graph (which provides the factorization that determines the coalition), we also evaluate the attribution when the graph is misspecified. In this case, the coalition will consist of $\{\cD_Y, \cD_{X|Y}\}$. We include these attribution results in Appendix \ref{app:add_results_syn}, specifically, Figure  \ref{fig:app_synthetic_misspec}. In this case, as expected, both $\cD_Y$ and $\cD_{X|Y}$ are attributed the change in model performance (at varying levels depending on the magnitude of concept shift). While this may still be a meaningful attribution, knowledge of the causal graph provides a more succinct interpretation of system behavior.  

\section{Related Work}




\textbf{Identifying relevant distribution shifts.}
There has been extensive work that tests whether the data distribution has shifted (e.g. ones evaluated in \citet{rabanser2019failing}). Past work has proposed to identify sub-distributions (factors constituting the joint distribution as determined by a generative model for the data) that comprise the shift between two joint distributions and order them by their contribution to the shift \citep{budhathoki2021distribution}. However, as suggested before, the sub-distributions may have different influence on model performance. Even a small change in some (factors) may have a large effect on model performance (and vice-versa). %
Thus, a model developer has to filter distributions to identify ones that actually impact model performance (see Property 2.2 and Appendix \ref{app:synthetic}). Further, ~\citet{budhathoki2021distribution} focuses on changes to the joint distribution as measured by the KL-divergence, which requires assumptions on the class of distributions to leverage closed-form expressions of KL-divergence (such as exponential families), or non-parametric KL estimation which is challenging in high dimensions \citep{wang2005divergence, wang2006nearest}. %

Other approaches which aim to localize shifts to individual variables (conditional on the rest of the variables) do not provide a way to identify the ones relevant to performance \citep{kulinski2020detection}. In contrast to testing for shifts, \citet{podkopaev2022tracking} tests for changes in model performance when distribution changes in deployment. Recent work by \citet{wu2021performance} decomposes performance change to changes in only marginal distributions using Shapley value framework~\citep{lundberg2017unified}. However, the method as described is restricted to categorical variables. \citet{kulinski2022towards} propose a method for distribution shift explanation based on transport mappings, though their focus is still on how the distribution has shifted and not its impact on some downstream model. %
In parallel work, \citet{cai2023diagnosing} propose a method for attributing performance degradation to distribution shifts, but their decomposition is limited to $P(X)$ and $P(Y|X)$ and thus has limited granularity.
Finally, \citet{jung2022measuring} propose a framework for measuring causal contributions to expected change in outcomes using Shapley values. This work focuses on attributions to specific feature \textit{values}, by framing causal attribution as hard/do-interventions in a causal system. Further, they only examine the system in a single domain,  and focus on the expected causal effect on a target variable $Y$. On the other hand, our work can be considered to focus on attributing model performance change to \textit{mechanisms} by considering mechanism changes across domains as ``soft-interventions''. Further, our main goal is to attribute model performance change across two fixed domains where we have access to iid samples from both domains.

\textbf{Shapley values for attribution.}
Shapley value-based attribution has recently become popular for interpreting model predictions \citep{strumbelj2014explaining,lundberg2017unified,wang2021flow}. In most prior work, Shapley values have been leveraged for attributing a specific model prediction to the input features~\citep{sundararajan2020many}. Challenges to appropriately interpreting such attributions and desirable properties thereof have been extensively discussed in~\cite{janzing2020feature, kumar2021shapley}. In this work, we advance the use of Shapley values for interpreting model performance changes to individual distributions at the dataset level. 

\textbf{Detecting data partitions with low model performance.}
Recent work aims to find subsets of the dataset that have significantly worse (or better) performance \citep{deon2021spotlight,eyuboglu2022domino, jain2022distilling, park2023trak}. However, they do not study changes in the underlying data distribution. The work by \citet{ali2022lifecycle} describes a method to identify and localize a change in model performance, and is applicable under distribution shifts. %
The main difference in our work is the data representations used for attribution. Instead of identifying subsets of \textit{data} that are relevant to performance change, we find individual \textit{distributions} represented by causal mechanisms. %


==> paper_arXiv/notation.tex <==
\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\global\long\def\reals{\mathbb{R}}
\global\long\def\pr{\mathbb{P}}
\global\long\def\E{\mathbb{E}}
\global\long\def\bX{\textbf{X}}
\global\long\def\U{\mathcal{U}}
\global\long\def\F{\mathcal{F}}
\global\long\def\R{\mathcal{R}}
\global\long\def\V{V}
\global\long\def\X{X}
\global\long\def\perf{\text{Perf}}
\global\long\def\psrc{\cD^\text{source}}
\global\long\def\ptar{\cD^\text{target}}
\global\long\def\noscriptcand{\texttt{C}}
\global\long\def\cand{\texttt{C}_{\cD}}
\global\long\def\subcand{\widetilde{\texttt{C}}}
\global\long\def\pa{\text{parent}}
\global\long\def\val{\text{Val}}
\global\long\def\attr{\text{Attr}}
\global\long\def\p{\mathbb{P}}
\global\long\def\bigO{\mathcal{O}}

\global\long\def\ouralg{\texttt{Perf-Shapley}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\def\note#1{\textcolor{blue}{#1}}

\newcommand{\tabref}[1]{{Table}~\ref{#1}}
\newcommand{\thref}[1]{{Theorem}~\ref{#1}}
\newcommand{\asref}[1]{{Assumption}~\ref{#1}}
\newcommand{\aref}[1]{{Algorithm}~\ref{#1}}
\newcommand{\propref}[1]{{Proposition}~\ref{#1}}
\newcommand{\lemref}[1]{{Lemma}~\ref{#1}}
\newcommand{\corref}[1]{{Corollary}~\ref{#1}}
\newcommand{\chref}[1]{{Chapter}~\ref{#1}}

\def\etal{et\/ al.\/ }
\def\bydef{:=}
\def\th{{^{th}}}
\def\suchthat{\text{s.t.}}

\def\embed{\hookrightarrow}
\def\to{{\,\rightarrow\,}}
\def\kron{\otimes}
\def\had{\circ}
\def\ksum{\oplus}

\mathchardef\mhyphen="2D
\newcommand{\smallmat}[1]{\left[\begin{smallmatrix}#1\end{smallmatrix}\right]}
\newcommand{\smallmt}[1]{\begin{smallmatrix}#1\end{smallmatrix}}


\newcommand{\tvec}[1]{{\text{vec}(#1)}}
\newcommand{\mat}[1]{{\text{mat}(#1)}} %
\newcommand{\indicator}[1]{ {\mathsf{1}}_{\left[ {#1} \right] }}

\def\half{\frac{1}{2}}
\newcommand{\fracl}[1]{\frac{1}{#1}}
\providecommand{\abs}[1]{{$\left\lvert#1\right\rvert$}}
\providecommand{\trans}[1]{{#1^\top}}
\providecommand{\inv}[1]{{#1^{-1}}}
\providecommand{\inner}[2]{{$\left\langle#1, #2\right\rangle$}}
\providecommand{\innere}[2]{{\trans{#1}#2}}
\providecommand{\innerd}[2]{{#1{\boldsymbol{\cdot}}#2}}
\providecommand{\brac}[1]{{$\left(#1\right)$}}

\providecommand{\dot}[2]{{\trans{#1}#2}}
\newcommand{\tr}[1]{{\mathrm{tr}}\!\left( #1 \right)}
\newcommand{\kl}[2]{{\mathrm{KL}\!\left({#1}\Vert{#2}\right)}}
\newcommand{\Hp}[1]{{\mathrm{H}\!\left({#1}\right)}}
\newcommand{\Hpp}[1]{-\Hp{#1}}

\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\newcommand{\normb}[1]{\norm{#1}_2}
\newcommand{\normbs}[1]{\normb{#1}^2}

\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\newcommand{\normf}[1]{\vertiii{#1}_2}
\newcommand{\normfs}[1]{\normf{#1}^2}
\newcommand{\normt}[1]{\vertiii{#1}_1}
\newcommand{\normr}[1]{\vertiii{#1}_0}

\newcommand{\normh}[2]{\vertiii{#1}_{2 \mhyphen #2}}
\newcommand{\normhs}[2]{\normh{#1}{#2}^2}
\newcommand{\normht}[2]{\vertiii{#1}_{1 \mhyphen #2}}
\newcommand{\normhr}[2]{\vertiii{#1}_{0\,\mhyphen #2}}

\newcommand{\gp}[2]{\cG\cP \left(#1, #2\right)}
\newcommand{\gpv}[3]{\cM\cG\cP \left(#1, #2, #3\right)}
\newcommand{\g}[2]{\cN\left(#1, #2\right)}
\newcommand{\gv}[3]{\cM\cN \left(#1, #2, #3\right)}
\newcommand{\etr}[1]{\text{etr}\left( #1 \right)}
\newcommand{\ev}[2]{\mathrm{E}_{ #1}\left[ \, #2 \, \right]}
\newcommand{\expf}[1]{ \exp \left( #1 \right) }
\newcommand{\exf}[1]{ e^{ #1 } }
\def\sut{\text{s.t.}}


\newcommand{\D}[2]{\frac{d #1}{d #2}} %
\newcommand{\dd}[2]{\frac{d^2 #1}{d #2^2}} %
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\gradb}[1]{\gv{\nabla} #1}
\newcommand{\grad}[1]{ \nabla_{#1} }

\newcommand{\vect}[1]{{\boldsymbol{#1}}}
\def\eps{\epsilon}
\def\balpha{\vect{\alpha}}
\def\bbeta{\vect{\beta}}
\def\bmu{\vect{\mu}}
\def\bnu{\vect{\nu}}
\def\beps{\vect{\epsilon}}
\def\bphi{\vect{\phi}}
\def\bpsi{\vect{\psi}}
\def\btheta{\vect{\theta}}
\def\bpi{\vect{\pi}}
\def\bgamma{\vect{\gamma}}
\def\beeta{\vect{\eta}}
\def\blambda{\vect{\lambda}}
\def\bkappa{\vect{\kappa}}
\def\bupsilon{\vect{\upsilon}}
\def\bomega{\vect{\omega}}
\def\btau{\vect{\tau}}
\def\brho{\vect{\rho}}
\def\bchi{\vect{\chi}}
\def\bPi{\vect{\Pi}}
\def\bPsi{\vect{\Psi}}
\def\bPhi{\vect{\Phi}}
\def\bTheta{\vect{\Theta}}
\def\bSigma{\vect{\Sigma}}
\def\bLambda{\vect{\Lambda}}
\def\bOmega{\vect{\Omega}}
\def\bDelta{\vect{\Delta}}
\def\bUpsilon{\vect{\Upsilon}}
\def\bAlpha{\vect{\vA}}
\def\bGamma{\vect{\Gamma}}
\def\bAlpha{\vect{A}}


\def\ba{{\mathbf{a}}}
\def\bb{{\mathbf{b}}}
\def\bc{{\mathbf{c}}}
\def\bd{{\mathbf{d}}}
\def\bee{{\mathbf{e}}}
\def\bff{{\mathbf{f}}}
\def\bg{{\mathbf{g}}}
\def\bh{{\mathbf{h}}}
\def\bi{{\mathbf{i}}}
\def\bj{{\mathbf{j}}}
\def\bk{{\mathbf{k}}}
\def\bl{{\mathbf{l}}}
\def\bm{{\mathbf{m}}}
\def\bn{{\mathbf{n}}}
\def\bo{{\mathbf{o}}}
\def\bp{{\mathbf{p}}}
\def\bq{{\mathbf{q}}}
\def\br{{\mathbf{r}}}
\def\bs{{\mathbf{s}}}
\def\bt{{\mathbf{t}}}
\def\bu{{\mathbf{u}}}
\def\bv{{\mathbf{v}}}
\def\bw{{\mathbf{w}}}
\def\bx{{\mathbf{x}}}
\def\by{{\mathbf{y}}}
\def\bz{{\mathbf{z}}}
\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}

\def\aa{{\vec{\ba}}}
\def\ab{{\vec{\bb}}}
\def\ac{{\vec{\bc}}}
\def\ad{{\vec{\bd}}}
\def\aee{{\vec{\be}}}
\def\aff{{\vec{\bf}}}
\def\ag{{\vec{\bg}}}
\def\ah{{\vec{\bh}}}
\def\ai{{\vec{\bi}}}
\def\ak{{\vec{\bk}}}
\def\al{{\vec{\bl}}}
\def\am{{\vec{\bm}}}
\def\an{{\vec{\bn}}}
\def\ao{{\vec{\bo}}}
\def\ap{{\vec{\bp}}}
\def\aq{{\vec{\bq}}}
\def\ar{{\vec{\br}}}
\def\as{{\vec{\bs}}}
\def\at{{\vec{\bt}}}
\def\au{{\vec{\bu}}}
\def\av{{\vec{\bv}}}
\def\aw{{\vec{\bw}}}
\def\ax{{\vec{\bx}}}
\def\ay{{\vec{\by}}}
\def\az{{\vec{\bz}}}
\def\aA{{\vec{\bA}}}
\def\aB{{\vec{\bB}}}
\def\aC{{\vec{\bC}}}
\def\aD{{\vec{\bD}}}
\def\aE{{\vec{\bE}}}
\def\aF{{\vec{\bF}}}
\def\aG{{\vec{\bG}}}
\def\aH{{\vec{\bH}}}
\def\aI{{\vec{\bI}}}
\def\aJ{{\vec{\bJ}}}
\def\aK{{\vec{\bK}}}
\def\aL{{\vec{\bL}}}
\def\aM{{\vec{\bM}}}
\def\aN{{\vec{\bN}}}
\def\aO{{\vec{\bO}}}
\def\aP{{\vec{\bP}}}
\def\aQ{{\vec{\bQ}}}
\def\aR{{\vec{\bR}}}
\def\aS{{\vec{\bS}}}
\def\aT{{\vec{\bT}}}
\def\aU{{\vec{\bU}}}
\def\aV{{\vec{\bV}}}
\def\aW{{\vec{\bW}}}
\def\aX{{\vec{\bX}}}
\def\aY{{\vec{\bY}}}
\def\aZ{{\vec{\bZ}}}

\def\bba{{\mathbb{a}}}
\def\bbb{{\mathbb{b}}}
\def\bbc{{\mathbb{c}}}
\def\bbd{{\mathbb{d}}}
\def\bbee{{\mathbb{e}}}
\def\bbff{{\mathbb{f}}}
\def\bbg{{\mathbb{g}}}
\def\bbh{{\mathbb{h}}}
\def\bbi{{\mathbb{i}}}
\def\bbj{{\mathbb{j}}}
\def\bbk{{\mathbb{k}}}
\def\bbl{{\mathbb{l}}}
\def\bbm{{\mathbb{m}}}
\def\bbn{{\mathbb{n}}}
\def\bbo{{\mathbb{o}}}
\def\bbp{{\mathbb{p}}}
\def\bbq{{\mathbb{q}}}
\def\bbr{{\mathbb{r}}}
\def\bbs{{\mathbb{s}}}
\def\bbt{{\mathbb{t}}}
\def\bbu{{\mathbb{u}}}
\def\bbv{{\mathbb{v}}}
\def\bbw{{\mathbb{w}}}
\def\bbx{{\mathbb{x}}}
\def\bby{{\mathbb{y}}}
\def\bbz{{\mathbb{z}}}
\def\bbA{{\mathbb{A}}}
\def\bbB{{\mathbb{B}}}
\def\bbC{{\mathbb{C}}}
\def\bbD{{\mathbb{D}}}
\def\bbE{{\mathbb{E}}}
\def\bbF{{\mathbb{F}}}
\def\bbG{{\mathbb{G}}}
\def\bbH{{\mathbb{H}}}
\def\bbI{{\mathbb{I}}}
\def\bbJ{{\mathbb{J}}}
\def\bbK{{\mathbb{K}}}
\def\bbL{{\mathbb{L}}}
\def\bbM{{\mathbb{M}}}
\def\bbN{{\mathbb{N}}}
\def\bbO{{\mathbb{O}}}
\def\bbP{{\mathbb{P}}}
\def\bbQ{{\mathbb{Q}}}
\def\bbR{{\mathbb{R}}}
\def\bbS{{\mathbb{S}}}
\def\bbT{{\mathbb{T}}}
\def\bbU{{\mathbb{U}}}
\def\bbV{{\mathbb{V}}}
\def\bbW{{\mathbb{W}}}
\def\bbX{{\mathbb{X}}}
\def\bbY{{\mathbb{Y}}}
\def\bbZ{{\mathbb{Z}}}
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}
\def\sfa{{\mathsf{a}}}
\def\sfb{{\mathsf{b}}}
\def\sfc{{\mathsf{c}}}
\def\sfd{{\mathsf{d}}}
\def\sfee{{\mathsf{e}}}
\def\sfff{{\mathsf{f}}}
\def\sfg{{\mathsf{g}}}
\def\sfh{{\mathsf{h}}}
\def\sfi{{\mathsf{i}}}
\def\sfj{{\mathsf{j}}}
\def\sfk{{\mathsf{k}}}
\def\sfl{{\mathsf{l}}}
\def\sfm{{\mathsf{m}}}
\def\sfn{{\mathsf{n}}}
\def\sfo{{\mathsf{o}}}
\def\sfp{{\mathsf{p}}}
\def\sfq{{\mathsf{q}}}
\def\sfr{{\mathsf{r}}}
\def\sfs{{\mathsf{s}}}
\def\sft{{\mathsf{t}}}
\def\sfu{{\mathsf{u}}}
\def\sfv{{\mathsf{v}}}
\def\sfw{{\mathsf{w}}}
\def\sfx{{\mathsf{x}}}
\def\sfy{{\mathsf{y}}}
\def\sfz{{\mathsf{z}}}
\def\sfA{\mathsf{A}}
\def\sfB{\mathsf{B}}
\def\sfC{\mathsf{C}}
\def\sfD{\mathsf{D}}
\def\sfE{\mathsf{E}}
\def\sfF{\mathsf{F}}
\def\sfG{\mathsf{G}}
\def\sfH{\mathsf{H}}
\def\sfI{\mathsf{I}}
\def\sfJ{\mathsf{J}}
\def\sfK{\mathsf{K}}
\def\sfL{\mathsf{L}}
\def\sfM{\mathsf{M}}
\def\sfN{\mathsf{N}}
\def\sfO{\mathsf{O}}
\def\sfP{\mathsf{P}}
\def\sfQ{\mathsf{Q}}
\def\sfR{\mathsf{R}}
\def\sfS{\mathsf{S}}
\def\sfT{\mathsf{T}}
\def\sfU{\mathsf{U}}
\def\sfV{\mathsf{V}}
\def\sfW{\mathsf{W}}
\def\sfX{\mathsf{X}}
\def\sfY{\mathsf{Y}}
\def\sfZ{\mathsf{Z}}
\def\fra{{\mathfrak{a}}}
\def\frb{{\mathfrak{b}}}
\def\frc{{\mathfrak{c}}}
\def\frd{{\mathfrak{d}}}
\def\free{{\mathfrak{e}}}
\def\frff{{\mathfrak{f}}}
\def\frg{{\mathfrak{g}}}
\def\frh{{\mathfrak{h}}}
\def\fri{{\mathfrak{i}}}
\def\frj{{\mathfrak{j}}}
\def\frk{{\mathfrak{k}}}
\def\frl{{\mathfrak{l}}}
\def\frm{{\mathfrak{m}}}
\def\frn{{\mathfrak{n}}}
\def\fro{{\mathfrak{o}}}
\def\frp{{\mathfrak{p}}}
\def\frq{{\mathfrak{q}}}
\def\frr{{\mathfrak{r}}}
\def\frs{{\mathfrak{s}}}
\def\frt{{\mathfrak{t}}}
\def\fru{{\mathfrak{u}}}
\def\frv{{\mathfrak{v}}}
\def\frw{{\mathfrak{w}}}
\def\frx{{\mathfrak{x}}}
\def\fry{{\mathfrak{y}}}
\def\frz{{\mathfrak{z}}}
\def\frA{\mathfrak{A}}
\def\frB{\mathfrak{B}}
\def\frC{\mathfrak{C}}
\def\frD{\mathfrak{D}}
\def\frE{\mathfrak{E}}
\def\frF{\mathfrak{F}}
\def\frG{\mathfrak{G}}
\def\frH{\mathfrak{H}}
\def\frI{\mathfrak{I}}
\def\frJ{\mathfrak{J}}
\def\frK{\mathfrak{K}}
\def\frL{\mathfrak{L}}
\def\frM{\mathfrak{M}}
\def\frN{\mathfrak{N}}
\def\frO{\mathfrak{O}}
\def\frP{\mathfrak{P}}
\def\frQ{\mathfrak{Q}}
\def\frR{\mathfrak{R}}
\def\frS{\mathfrak{S}}
\def\frT{\mathfrak{T}}
\def\frU{\mathfrak{U}}
\def\frV{\mathfrak{V}}
\def\frW{\mathfrak{W}}
\def\frX{\mathfrak{X}}
\def\frY{\mathfrak{Y}}
\def\frZ{\mathfrak{Z}}

\def \ttS{\texttt{S}}

